Time Waits for No One! Analysis and Challenges of Temporal Misalignment

When an NLP model is trained on text data from one time period and tested or deployed on data from another, the resulting temporal misalignment can degrade end-task performance. In this work, we establish a suite of eight diverse tasks across different domains (social media, science papers, news, and reviews) and periods of time (spanning five years or more) to quantify the effects of temporal misalignment. Our study is focused on the ubiquitous setting where a pretrained model is optionally adapted through continued domain-specific pretraining, followed by task-specific finetuning. We establish a suite of tasks across multiple domains to study temporal misalignment in modern NLP systems. We find stronger effects of temporal misalignment on task performance than have been previously reported. We also find that, while temporal adaptation through continued pretraining can help, these gains are small compared to task-specific finetuning on data from the target time period. Our findings motivate continued research to improve temporal robustness of NLP models.

==> Temporal Drift Analysis(3)/dapt_table_old.tex <==
\begin{table*}[]
    \centering
% \includegraphics[width=0.9\textwidth]{tables/GPT2_twitter_dapt_downstream.png}
% \includegraphics[width=0.75\textwidth,trim=7.9cm 7cm 1cm 0cm]{"tables/Temporal Drift - GPT2 DAPT.pdf"}
% \includegraphics[width=1.0\linewidth,trim=1.70cm 11.1cm 10.7cm 1.8cm,clip=true]{figures/gpt2-twitter-dapting-the-one!!.pdf}
% \includegraphics[width=0.98\linewidth,trim=0.6cm 4.99cm 11.3cm 1.87cm,clip=true]{figures/gpt2-dapting-the-one!!-2.pdf}
% \includegraphics[width=0.99\linewidth,trim=2.34cm 9.99cm 15.7cm 1.86cm,clip=true]{tables/gpt2-dapting-the-one!!-5.pdf}
\includegraphics[width=0.99\textwidth,trim=0.8cm 22.6cm 1.5cm 1.5cm]{tables/gpt-dapt-compressed.pdf}
%\includegraphics[width=0.99\pagewidth,trim=0.8cm 10.6cm 18.95cm 1.9cm,clip=true]{tables/gpt2-dapting-the-one!!-5.pdf}
\caption{Combination of temporal adaptation and finetuning  (\S\ref{subsub:adaptaton:plus:tuning})  on our tasks. 
% evaluated in terms of classification F1. 
The row labeled ``Default'' corresponds to a model that has not been adapted (uses the default pretraining). 
% - (1) political party prediction based on tweets (Twitter), controversy prediction on the nba subreddit (Reddit), and MESH tagging on scientific articles (Science). 
% they \daniel{?} can be found in \S\ref{table:gpt2_twitter_downstream}.
The color coding is proportional to the magnitude of the performances of each task (darker shade of \orangetext{orange} indicates higher scores). 
We see that models that were finetuned on similar time periods performed similarly, no matter how their DAPT conditions differed.
% It can be observed that the two top-left and bottom-right quadrants of each tasks (corresponding to synchronous finetuning) 
% \daniel{TODO}\kelvin{is there an elegant way to heatmap tables? There is: I'll update this and do it on Monday}
}
\label{table:gpt2_dapt}
\end{table*}

==> Temporal Drift Analysis(3)/dataset.tex <==
\begin{table*}[t]
    \small 
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ccccm{10cm}}
        \toprule
            Domain & Task & Time Range & Size & Example \\ 
        \midrule
            \multirow{3}{*}{Twitter}  & \makecell{political\\affiliation\\classification} & 2015-2019 & $120k$ &  \textbf{Input:} \emph{History will note that Trump didn’t merely fiddle while the planet burned but tried to throw the Arctic National W... } \textbf{Output:} \emph{Democrat (vs Republican) }  \\ 
            % \specialrule{.001em}{.001em}{.001em} 
            \cline{2-5}
            & \makecell{entity type\\classification} & 2014-2019 & $8k$  &  \textbf{Input:} \emph{entity: Finola, tweet: Two 64-year olds enjoying their first birthday together in 40+ years. My twin sister, Finola, and I.}    \textbf{Output:} \emph{Person}  \\ 
            \specialrule{.001em}{.001em}{.001em} 
            % Reddit & \makecell{popularity\\detection} & 2014-2019 & ? & \textbf{Input:} In general, I feel young players, potential, and lottery picks are overrated. ... \textbf{Output:} controversial \daniel{needs to be updated} \\
            \specialrule{.001em}{.001em}{.001em} 
            \multirow{4}{*}{Science} & \makecell{mention\\type\\classification} & 1980-2016 & $8k$ &   \textbf{Input:}  \emph{mention: deep Long Short-Term Memory (LSTM) subnetwork, abstract: In this paper, we study the problem of online action detection from the streaming skeleton data .... by leveraging the merits of the deep Long Short-Term Memory (LSTM) subnetwork, the proposed model ...} \textbf{Output:} \emph{Method}  \\
            % \specialrule{.001em}{.001em}{.001em} 
            \cline{2-5}
             & \makecell{venue\\classification} & 2009-2020 & $16k$ & \textbf{Input:} \emph{Rank K Binary Matrix Factorization (BMF) approximates a binary matrix by the product of two binary matrices of lower rank, K...}  \textbf{Output:} \emph{AAAI (vs ICML)} \\ 
            \specialrule{.001em}{.001em}{.001em} 
            \multirow{7}{*}{News} & \makecell{media \\ frame\\classification} & 2009-2016 & $20k$ & \textbf{Input:} \emph{You think you have heard the worst horror a gun in the wrong hands can do, and then this.You think there could not have been anywhere more tragic for it to happen...}  \textbf{Output:} \emph{Gun Control (15 possible frames)} \\ 
            % \specialrule{.001em}{.001em}{.001em} 
            \cline{2-5}
             & \makecell{publisher \\ classification} & 2009-2016 & 67$k$ & \textbf{Input:} \emph{A Muslim woman said Sunday that her viral article explaining why she voted for Donald Trump has angered her liberal pals as well as other Muslims.}  \textbf{Output:} \emph{FoxNews (vs NYTimes or WaPost)} \\ 
            % \specialrule{.001em}{.001em}{.001em} 
            \cline{2-5}
             & \makecell{summarization} & 2009-2016 & 330$k$ & \textbf{Input:} \emph{The Consumer Financial Protection Bureau is demanding PayPal return \$15 million to consumers and pay a \$10 million fine for ...}  \textbf{Output:} \emph{The CFPB alleges many customers unwittingly signed up for PayPal Credit} \\ 
             \specialrule{.001em}{.001em}{.001em}
             Food Reviews & \makecell{review rating \\ classification} & 2013-2019 & $126k$ & \textbf{Input:} \emph{What a beautiful store and amazing experience! Not only the atmosphere, but the people...}  \textbf{Output: } \emph{4 (out of 5)} \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{The tasks from four domains studied in this paper, with examples. See Section~\ref{subsec:datasets} for more details. 
    % \suchin{If we are looking to cut, we can remove the examples (or move them to appendix). we  should point readers to section 3.4 for task descriptions. }
    % As it can be seen, a variety of domains are covered in this work.
    }
    \label{tab:task:examples}
\end{table*}

==> Temporal Drift Analysis(3)/ft_tdscore_table.tex <==
\begin{table}[t]
\centering
\small


\pgfplotstabletypeset[
    typeset cell/.append code={%
    \ifx#1\pfft%
    \pgfkeyssetvalue{/pgfplots/table/@cell content}{\\ \midrule}%
    \fi},
    columns={Z,A,B,C, dummy},
    col sep=comma, 
    every head row/.style={before row=\toprule, after row=\midrule },
    %every first row/.style={after row=\bottomrule},
    every last row/.style={after row=\bottomrule},
    %columns/Domain/.style={reset styles},
    % columns/Task/.style={reset styles},
    columns/Z/.style={ reset styles, string type,
    column name={Domain}, column type={l}},
    columns/A/.style={reset styles, string type, , column name=Task (metric), column type={|l}},
    columns/B/.style={ column name=TD,fixed zerofill, column type={|l}},
    %columns/C/.style={ round-precision=2, round-mode=places, column name=$r$, fixed zerofill},
    columns/C/.style={ column name=$r$, fixed zerofill},
    columns/dummy/.style={string type,column name={}}
]{table.dat}
    \caption{
        Finetuned models' temporal degradation summary scores (TD; \S\ref{subsec:metric}; details in Figure~\ref{table:gpt2_downstream_tasks}). 
        These scores estimate how fast a model degrades as the time period of training and evaluation data diverge (higher scores imply faster degradation). We note that since we normalize by the overall time range of a task, the temporal partitions we used do have an effect on the TD scores. For example, \ai{} spans ten years, even though there are only four partitions.
        \added{We also show the correlation coefficient, $r$, that measures the strength of a linear relationship (0 meaning no correlation, 1 being perfectly correlated). In all cases but Yelp, the degree of degradation has a moderate correlation with the distance between the training and evaluation years ($r>0.5$, $p<0.05$). We use the Wald test with the null hypothesis that the slope is 0. }
    }
    \label{tab:td:scores:fine-tuned} 
\end{table}


==> Temporal Drift Analysis(3)/heatmap_results.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/finetuning/heatmap_results.png}
\caption{
    Temporal misalignment in finetuning affects task performance (\S\ref{subsub:finetuning}). In all cases, higher scores are better. The heatmap is shaded per column, i.e., the darkest shade of \orangetext{orange} in a cell means the cell has the highest score in that column.
    % measured in terms of classification F1. 
    % Political party prediction based on tweets (GPT2).
    % Being evaluated on a
    Mismatch between the the training and evaluation data can result in massive performance drop; degree varies by task.
For example, \yelpreview{}, \mediaframes{}, and \twiet{} show minimal degradation. In contrast, \poliaff{} and \summarization{} major deterioration over time. 
}
\label{figure:gpt2_downstream_tasks_all}
\end{figure*}


==> Temporal Drift Analysis(3)/label_distr.tex <==
\begin{figure}
\centering
\includegraphics[width=.5\textwidth,trim=0cm 0cm 0cm 0.9cm]{figures/overlap_figures/label_distr.png}
\caption{
    KL divergence between label distributions over time for all tasks. For each cell, we compare the distribution of labels to that of the first time period; e.g., the 2017 \poliaff{} cell contains the KL-divergence between the label distributions of \poliaff{} in 2017 and 2015. We note that while most distributions see little change over time, \poliaff{}, \ai{} and \mediaframes{} see a large shift. However, we note that \poliaff{} was sensitive to temporal misalignment while \mediaframes{} was not. 
}
\label{figure:label_distr}
\end{figure}


==> Temporal Drift Analysis(3)/label_distr_subs.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.4\textwidth,trim=0cm 0.4cm 0cm 0.3cm]{figures/overlap_figures/label_distr_subs.png}
\caption{
    KL divergence between label distributions over time for a subset of tasks. See Appendix~\ref{sec:appendixB} for full results. For each cell, we compare the distribution of labels to that of the first time period; e.g., the 2017 \poliaff{} cell contains the KL-divergence between the label distributions of \poliaff{} in 2017 and 2015. While most tasks see little change over time, \poliaff{} and \mediaframes{} see a large shift. %However, \poliaff{} was sensitive to temporal misalignment while \mediaframes{} was not. 
}
\label{figure:label_distr_subs}
\end{figure}


==> Temporal Drift Analysis(3)/overlapcorr.tex <==
\begin{table}
\centering
\small


\pgfplotstabletypeset[
    typeset cell/.append code={%
    \ifx#1\pfft%
    \pgfkeyssetvalue{/pgfplots/table/@cell content}{\\ \midrule}%
    \fi},
    columns={Z,A,B,dummy},
    col sep=comma, 
    every head row/.style={before row=\toprule, after row=\midrule },
    %every first row/.style={after row=\bottomrule},
    every last row/.style={after row=\bottomrule},
    %columns/Domain/.style={reset styles},
    % columns/Task/.style={reset styles},
    columns/Z/.style={ reset styles, string type,
    column name={Domain}, column type={l}},
    columns/A/.style={reset styles, string type, , column name=Task (metric), column type={|l}},
    columns/B/.style={ column name=Pearson's $r$,fixed zerofill, column type={|l}},
    %columns/C/.style={ round-precision=2, round-mode=places, column name=$r$, fixed zerofill},
        columns/C/.style={ column name=$r$, fixed zerofill},
    columns/dummy/.style={string type,column name={}}
]{table2.dat}
    \caption{
    \added{        Pearson $r$ correlation coeffecients between the word overlap and performance of each task. }
    }
    \label{tab:overlapcorr} 
\end{table}


==> Temporal Drift Analysis(3)/pretrain_heatmap.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=.38\textwidth,trim=1.9cm .5cm 1.0cm 0.9cm]{figures/pretrain/pretrain_heatmap.png}
\caption{
    Perplexity of GPT2 after adaptive pretraining on temporally-selected data in different domains (lower is better). The TD score (in parentheses) estimates the expected perplexity rise (i.e., degradation) for every time period of misalignment between evaluation and training times.  Degradation follows the expected pattern, but the magnitude varies by domain. 
    % even a minor one in the Yelp domain where we did not expect any shift. 
  %  \kelvin{. Does this highlight what we want to show actually? Notably for newsroom - we want to emphasize a sense of regret rather than actual degradation? Should we color code by column, rather than row? (and make it clear in the caption)?}
   % \suchin{We should be clear in the figure (maybe title of each heatmap?) that this is perplexity and not F1. }
}
\label{figure:gpt2_lm}
\end{figure}


==> Temporal Drift Analysis(3)/small_heatmap.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.95\textwidth,trim=0cm .35cm 0cm 0.5cm]{figures/finetuning/small_heatpmap.png}
\caption{
    Temporal misalignment in finetuning affects task performance (\S\ref{subsub:finetuning}). In all cases, higher scores are better. The heatmap is shaded per column, i.e., the darkest shade of \orangetext{orange} in a cell means the cell has the highest score in that column.
    % measured in terms of classification F1. 
    % Political party prediction based on tweets (GPT2).
    % Being evaluated on a
    Mismatch between the the training and evaluation data can result in massive performance drop; the degree varies by task. 
%    While all suffer from temporal degradation, its degree is a strong function of task definition. 
    For example, \yelpreview{} shows minimal degradation. In contrast, \poliaff{} shows major deterioration over time. Additional tables for remaining tasks can be found in Appendix \ref{sec:appendixB}.
    %\kelvin{TODO: Make fonts bigger still?}
    %\suchin{We should be clear in the figure (maybe title of each heatmap?) that this is F1 and not perplexity. }
    % \daniel{I think you have room to spell out "R-L".}
å}
\label{table:gpt2_downstream_tasks}
\end{figure*}


==> Temporal Drift Analysis(3)/td_score_more.tex <==
\begin{figure*}
\centering
\includegraphics[trim=0cm 0.6cm 0cm 0cm, width=\textwidth]{figures/other/td_more.png}
\caption{
    Three example calculations of the TD score (left from \poliaff{} and the center and right from \yelpreview{}). The annotated numbers are the raw evaluation scores $S_{t'\to t}$ and the plotted markers represent the modified differences $D(t'\to t)$ discussed in Section~\ref{subsec:metric}. For a particular plot, the red line is the line of best fit and its slope is the $\text{TD}(t)$ score for evaluation timestep $t$. The final TD score is averaged between all evaluation timesteps for the particular task.
}
\label{figure:td_more}
\end{figure*}


==> Temporal Drift Analysis(3)/td_score_plot.tex <==
\begin{figure}
\centering
\includegraphics[trim=0.5cm 0.5cm 0cm 0cm, width=.35\textwidth]{figures/other/td_score.png}
\caption{
    An example calculation of the TD score for a particular timestep $t$ (discussed in Section~\ref{subsec:metric}).
        The plotted markers represent $D(t'\to t)$ ($y$-axis) as a function of train time period $t'$  ($x$-axis). 
        The annotated numbers on each blue dot are the raw evaluation scores $S_{t'\to t}$, not to be confused with the $y$ values.
    The red line is the line of best fit and its slope is the TD score for evaluation timestep $t$. In this example, we would expect to see, on average, $9.09$ points of deterioration for each year of misalignment. The final TD score is averaged across all evaluation timesteps. 
}
\label{figure:td_example}
\end{figure}


==> Temporal Drift Analysis(3)/word_overlap.tex <==
\begin{figure*}[t]
\centering
\includegraphics[trim=0cm 0.6cm 0cm 0cm, width=\textwidth]{figures/overlap_figures/domain_word_overlap_scaled}
\caption{
    Vocabulary overlap between time periods, over a subset of our tasks' datasets. Each cell shows the \% overlap between the vocabularies of two time periods.} %We find vocabularies using the evaluation sets and compare the most frequent 10K unigrams between training sets. }
\label{figure:word_overlap}
\end{figure*}


==> label_distr.tex <==
\begin{figure}
\centering
\includegraphics[width=.5\textwidth,trim=0cm 0cm 0cm 0.9cm]{figures/overlap_figures/label_distr.png}
\caption{
    KL divergence between label distributions over time for all tasks. For each cell, we compare the distribution of labels to that of the first time period; e.g., the 2017 \poliaff{} cell contains the KL-divergence between the label distributions of \poliaff{} in 2017 and 2015. We note that while most distributions see little change over time, \poliaff{}, \ai{} and \mediaframes{} see a large shift. However, we note that \poliaff{} was sensitive to temporal misalignment while \mediaframes{} was not. 
}
\label{figure:label_distr}
\end{figure}

